Beyond Node Degree: Evaluating AS Topology Models

Many models have been proposed to generate Internet Autonomous System (AS) topologies, most of which make structural assumptions about the AS graph. In this paper we compare AS topology generation models with several observed AS topologies. In contrast to most previous works, we avoid making assumptions about which topological properties are important to characterize the AS topology. Our analysis shows that, although matching degree-based properties, the existing AS topology generation models fail to capture the complexity of the local interconnection structure between ASs. Furthermore, we use BGP data from multiple vantage points to show that additional measurement locations significantly affect local structure properties, such as clustering and node centrality. Degree-based properties, however, are not notably affected by additional measurements locations. These observations are particularly valid in the core. The shortcomings of AS topology generation models stems from an underestimation of the complexity of the connectivity in the core caused by inappropriate use of BGP data.

==> Makefile <==
###########################################################
#
# Makefile for LaTeX docs
#
# $Id: 
#

.SUFFIXES:
.SUFFIXES: .ps .dvi .tex

TEXINPUTS := .:${TEXINPUTS}
BIBINPUTS := .:${TEXINPUTS}

TEX = $(wildcard *.tex)
all: eps dvi ps pdf
eps: fig obj

ps:  sigcomm2k8.ps  eps
pdf: sigcomm2k8.pdf eps
dvi: sigcomm2k8.dvi eps

obj: $(patsubst %.obj, %.eps, $(wildcard *.obj))
fig: $(patsubst %.fig, %.eps, $(wildcard *.fig))

clean:
	$(RM) *.aux *.log *.bbl *.blg *~ \#*\# *.toc *.idx
	$(RM) $(patsubst %.tex, %.ps, $(wildcard *.tex))
	$(RM) $(patsubst %.tex, %.dvi, $(wildcard *.tex))
	$(RM) $(patsubst %.tex, %.pdf, $(wildcard *.tex))

distclean: clean
	$(RM) $(patsubst %.fig, %.eps, $(wildcard *.fig))
	$(RM) $(patsubst %.obj, %.eps, $(wildcard *.obj))

# only need -Ppdf if using CM fonts

%.pdf: %.dvi $(wildcard *.bib)
	dvips -Ppdf -G0 -t letter -o $*.tmp.ps $<
	ps2pdf -dEmbedAllFonts=true -dSubsetFonts=true -dEPSCrop=true $*.tmp.ps $*.pdf
	$(RM) $*.tmp.ps
#	$(RM) $*.tmp.ps $*.dvi *.aux *.log *.bbl *.blg *.toc

%.dvi: $(TEX) $(wildcard *.bib)
	latex $*
	bibtex $*
	if [ -e $*.toc ] ; then bibtex $*; latex $* ; fi
	if [ -e $*.bbl ] ; then bibtex $*; latex $* ; fi
	if egrep Citation $*.log ; then bibtex $*; latex $*; fi
	if egrep Citation $*.log ; then bibtex $*; latex $*; fi
	if egrep Rerun $*.log ; then latex $* ; fi
	if egrep Rerun $*.log ; then latex $* ; fi
	if egrep Rerun $*.log ; then latex $* ; fi

%.ps: %.dvi
	dvips -tletter -o $@ $<

%.ps.gz: %.ps
	gzip -v9 $<

%.eps: %.obj
	tgif -color -print -eps $*

%.eps: %.fig
	fig2dev -L eps $< $@

toc: $(wildcard *.tex)
	@egrep -h "\\\((sub)*section|chapter)" $+ | egrep -v "^%" | \
                sed -e 's/\\chapter//;                          \
                s/\\section/    /;                              \
                s/\\subsection/         /;                      \
                s/\\subsubsection/                      /;      \
                s/\\.*{//g;s/[{}]//g' > $@


==> abstract.tex <==
Many models have been proposed to generate Internet Autonomous System (AS) 
topologies, most of which make structural assumptions about the AS graph. 
In this paper we compare AS topology generation models with several observed 
AS topologies. In contrast to most previous works, we avoid making assumptions 
about which topological properties are important to characterize the AS topology.
Our analysis shows that, although matching degree-based properties, the existing 
AS topology generation models fail to capture the complexity of the local 
interconnection structure between ASs. Furthermore, we use BGP data from multiple
vantage points to show that additional measurement locations significantly 
affect local structure properties, such as clustering and node centrality. 
Degree-based properties, however, are not notably affected by additional measurements 
locations. These observations are particularly valid in the core. The shortcomings 
of AS topology generation models stems from an underestimation of the complexity 
of the connectivity in the core caused by inappropriate use of BGP data.

==> available.tex <==
\section{AS topology models}
\label{sec:tools}

There are many models available that claim to describe the Internet AS
topology. Several of these models are embodied in tools for generating
simulated topologies~\cite{hamedsurvey}. In this section we describe the particular
models whose output we compare in this paper.  The first are produced
from the Waxman model~\cite{waxman}, derived from the
Erd\"{o}s-R\'{e}nyi random graphs~\cite{random}, where the probability
of two nodes being connected is proportional to the Euclidean distance
between them. The second come from the Barabasi and Albert~\cite{ba}
model, following measurements of various power laws in degree
distributions and rank exponents by Faloutsos
\etal~\cite{powerlaw}. These incorporate common beliefs about
preferential attachment and incremental growth. The third are from the
Generalized Linear Preference model~\cite{bu} which additionally model
clustering coefficients. Finally, Inet~\cite{inet} and
PFP~\cite{shizhou} focus on alternative AS topology characteristics:
the meshed core and preferential attachment respectively. Each model
focused only on particular metrics and parameters, and only compared
their output with selected AS topology observations.

\subsection{Waxman}
The Waxman model of random graphs is based on a probability model for
interconnecting nodes of the topology given by: $\displaystyle P(u,v)
= \alpha$ $e^{-d/(\beta L)}$, where $\displaystyle 0 < \alpha ,\beta
\leq 1 $, $d$ is the Euclidean distance between two nodes $u$ and $v$,
and $L$ is the network diameter (largest distance between two nodes).
We use the BRITE~\cite{brite} implementation of this model in this
paper, which facilitates re-wiring using iterative assignment of edges
to ensure that there are no disconnected components in the generated
topology.

\subsection{BA}
The BA model was inspired by the idea of preferentially attaching new
nodes to existing well-connected nodes, leading to the incremental
growth of nodes and the links between them. When a node $i$ joins the
network, the probability that it connects to a node $j$ already in the
network is given by: $\displaystyle P(i,j) = \frac{d_{j}}{\sum_{k \in
V}{d_{k}}}$ where $d_{j}$ is the degree of node $j$, $V$ is the set of
nodes that have joined the network and $\sum_{k \in V}{d_{k}}$ is the
sum of degrees of all nodes that previously joined the
network~\cite{brite}.

\subsection{GLP}
Our third model is the Generalized Linear Preference model
(GLP)~\cite{bu}. This focuses on matching characteristic path length
and clustering coefficients. It uses a probabilistic method for adding
nodes and links recursively while preserving selected power law
properties.

\subsection{Inet}
Inet~\cite{inet} produces random networks using a preferential linear
weight for the connection probability of nodes after modelling the
core of the generated topology as a full mesh network. Inet sets the
minimum number of nodes at 3037, the number of ASs on the Internet at
the time of its development. It similarly sets the fraction of degree
1 nodes to 0.3, based on measurements from
Routeviews\footnote{\url{http://www.routeviews.org/}} and
NLANR\footnote{\url{http://www.nlanr.net/}} BGP table data in 2002.


\subsection{PFP}
In the Positive Feedback Preference (PFP) model, the AS topology of
the Internet is considered to grow by interactive, probabilistic
addition of new nodes and links. It uses a nonlinear preferential
attachment probability when choosing older nodes for the interactive
growth of the network, by inserting edges between existing nodes as
well as the newly added ones.


==> observed-topos.tex <==
\section{AS topology observations}
\label{sec:observed}

The Internet AS topology can be inferred from various sources of data
such as BGP or traceroute~\cite{traceroute} at the network (IP)
layer. Using BGP routing data alone suffers from incompleteness, no
matter how many vantage points are used to collect observations.  In
particular, even if BGP updates are collected from multiple vantage
points and combined, many peering and sibling relationships are not
observed~\cite{olaf}. Conversely, traceroute data misses alternative
paths since routers may have multiple interfaces which are not easily
identified, and multi-hop paths may also be hidden by traffic
tunnelled via Multi-Protocol Label Switching (MPLS).  Combining these
data sources still does not solve all problems since mapping
traceroute data to AS numbers is not always accurate~\cite{jennifer}.
In this paper we attempt to avoid these problems by comparing against
many measurement-derived datasets giving a diverse spatial and
temporal comparison across different continents and years of
measurement.

\subsection{Chinese} 
The first dataset is a traceroute measurement of the Chinese AS
Topology collected from servers within China in May 2005. It reports
84 ASs, representing a small subgraph of the Internet.
Zhou~\etal~\cite{chinese} maintain that the Chinese AS graph presents
all the major topology characteristics of the global AS graph. The
presence of this dataset enables us to compare the AS topology models
at smaller scales. Further, this dataset is believed to be nearly
complete, i.e.,~it contains very little measurement bias and
accurately represents the true AS topology for that region of the
Internet. Thus, although it is rather small, we have included it as a
valuable comparison point in our studies.

\subsection{Skitter} 
The second dataset comes from the CAIDA Skitter
project\footnote{\url{http://www.caida.org/tools/measurement/Skitter/}}.
CAIDA computes the adjacency matrix of the AS topology from the daily
Skitter measurements. These are obtained by running traceroutes over a
large range of IP addresses and mapping the prefixes to AS numbers
using RouteViews BGP data. Since this data reports paths actually
taken by packets, rather than path information propagated via BGP, it
more directly represents the IP topology than the BGP data alone.
%% From routing point of view, a downside to
%% the Skitter data is that since it represents paths that have actually
%% been traversed by packets to their destinations, rather than paths
%% calculated and propagated by BGP system, it is more likely to
%% faithfully represent the IP topology than the BGP data alone. 
For our study, we used the graphs for March 2004 as used by Mahadevan
\textit{et al.}~\cite{lessons}, which reports 9,204 unique ASs.

\subsection{RouteViews} 
The third dataset we use is derived from the RouteViews BGP data.
This is collected both as static snapshots of the BGP routing tables
and dynamic BGP data in the form of BGP update and withdrawal
messages. We use the topologies provided by Mahadevan \textit{et
al.}~\cite{lessons} from two types of BGP data from March 2004: one
from the static BGP tables and one from the BGP updates. In both
cases, they filter AS-sets and private ASs and merge the 31 daily
graphs into one. This dataset reports 17,446 unique ASs across 43
vantage points in the Internet.

% (across all $165,171$ observed prefixes\footnote{Note in May 2007 RouteViews had up to $46$ active vantage points, they observed $25,967$ ASs and a total of $258,636$ prefixes. There are also $62,709$ inter-AS links visible.}). 


\subsection{UCLA} 
The fourth dataset comes from the Internet topology
collection\footnote{\url{http://irl.cs.ucla.edu/topology/}} maintained
by Oliviera \textit{et al.}~\cite{asevolution}. These topologies are
updated daily using the data sources such as BGP routing tables and
updates from RouteViews,
RIPE\footnote{\url{http://www.ripe.net/db/irr.html}},
Abilene\footnote{\url{http://abilene.internet2.edu/}} and LookingGlass
servers. Each node and link is annotated with the times it was first
and last observed. We use a snapshot of this dataset from November
2007 computed using a time window on the last-seen timestamps to
discard ASs which have not been seen for more than 6 months. The
resulting dataset reports 28,899 unique ASs.




==> related.tex <==
\section{Related Work}
\label{sec:related}

Zegura \etal~\cite{zegura97quantitative} analyse topologies of 100
nodes generated using pure-random, Waxman~\cite{waxman}, exponential
and several locality based models of topology such as Transit-Stub.
They use metrics such as average node degree, network diameter, number
of paths between nodes. They find that pure random topologies
represent expected properties such as locality very poorly and so we
exclude them from our comparison. They suggest that the Transit-Stub
method should be used due both to its efficiency and the realistic
average node degree its topologies achieve.

Faloutsos \textit{et al.}~\cite{powerlaw} state that three specific
properties of the Internet AS topology are well described by power
laws: rank exponent, out-degree exponent and eigen-exponent (graph
eigenvalues). This work parallelled development of many models
incorporating power laws, such as the Barab\'{a}si and
Albert~\cite{ba} model, based on incremental growth by addition of new
nodes and preferential attachment of new nodes to existing
well-connected nodes.
%% In this paper we investigate the biases of
%% such models.

Later, Bu and Towsley~\cite{bu} used the empirical complementary
distribution (ECD) rather than standard histograms to generate new
nodes. They showed the variability in graphs from different generators
using the same heuristics using characteristic path length and
clustering coefficients.

Tangmunarunkit \textit{et al.}~\cite{degreebased} provide a first
comparison of the underlying characteristics of degree-based models
against structural models. A major conclusion is that the the simplest
form of degree-based model performs better than random or structural
models at representing the studied parameters. They compare three
categories of model generators: Waxman, Tiers~\cite{tiers} and the
Transit-Stub structural model, against the simplest degree based
generator, the power-law random graph (PLRG)~\cite{plrg}. They define
and use three metrics: expansion, resilience and distortion. They find
that the PLRG matches these metrics better than the random or
structural models. Based on these metrics they conclude that stricter
hierarchy is present in the measured networks than in degree-based
generators. However, they leave many questions unanswered about the
accuracy of degree-based generators and the choice of metrics.

Zhou and Mondragon~\cite{shizhou} propose models based on several
mathematical features, such as rich-club, interactive growth and
betweenness centrality. They use AS data from the CAIDA Skitter
project to examine the Joint Degree Distribution (JDD) and rich-club connectivity. They show that
for these data, rich-club connectivity and the JDD are closely linked
for a network with a given degree distribution.

In this paper, we consider more recent degree-based generators
using a larger set of graph-theory derived metrics to give better
insight into correct understanding of the AS topology. We 
 compare in detail against a range of different Internet AS topologies
at national and international level obtained from traceroute and BGP
data. When choosing our metrics, we considered both metrics used by
the topology generator designers and those used more widely in graph
theory. A particular point to note is that we chose not to use the
three metrics of Tangmunarunkit \etal{} for two reasons. First,
computation of both resilience and distortion are NP-complete,
requiring use of heuristics. In contrast, all our metrics are
straightforward to compute directly. Second, although accurate
reproduction of degree-based metrics is well-supported by current
topology generators, our hypothesis was that local interconnectivity
was poorly supported, and so we chose to use several metrics that
focus on exactly this, e.g.,~assortativity, clustering, and
centrality.


%this is not for internet.. what shall we do?

% Finally, Jamakovic \etal~\cite{Jamakovic} compare various metrics against real world networks such as railway lines, road infrastructure and power grid. They suggest some topological metrics tend to have stronger correlations with each other and hence may be redundant. However, in this paper we present an extensive set of metrics which have been used by the topology generator designers as well as graph theorists. 


==> topology.tex <==
\section{Topology characterization}
\label{sec:topology}

Over the past several years a veriety of topological metrics has been proposed
to quantitatively characterize topological properties of networks. In
this section we present a large set of topological metrics that will be used
to measure a \emph{distance} in graph space, i.e. how distant two graphs are
topologically from each other. The topological metrics are computed for
the synthetic and the measured AS topologies. Taken individually, these
metrics concentrate on differing topological aspects but when considered
together they reveal the shortcomings of topology models to faithfully capture
the topological properties of observed AS topologies. AS topologies are modeled
as graphs $G=(\mathcal{N},\mathcal{L})$ with a collection of nodes
$\mathcal{N}$ and a collection of links $\mathcal{L}$ that connect a pair of
nodes.\ The number of nodes and links in a graph is then respectively equal to
$N=\left\vert \mathcal{N}\right\vert $ and $M=\left\vert \mathcal{L}%
\right\vert $.

\subsection{Degree}

The degree $k$ of a node is the number of links adjacent to it. The
\emph{average node degree} $\bar{k}$ is defined as $\bar{k}=2M/N$. The
\emph{node degree distribution} $P(k)$ is the probability that a randomly
selected node has a given degree $k$. The node degree distribution is defined
as $P(k)=n(k)/N$ where $n(k)$ is the number of nodes of degree $k$. The
\emph{joint degree distribution} (JDD) $P(k,k^{\prime})$ is the probability
that a randomly selected pair of connected nodes have degrees $k$ and
$k^{\prime}$. A summary measure of the joint degree distribution is the
average neighbor degree of nodes with a given degree $k$, and is defined as
follows $k_{nn}(k)=\sum_{k^{\prime}=1}^{k_{max}}k^{\prime}P(k^{\prime}|k)$.
The maximum possible $k_{nn}(k)$ value is $N-1$ for a maximally connected
network, i.e. a complete graph. Hence, we represent JDD by the normalized
value $k_{nn}(k)/(N-1)$ \cite{lessons} and refer to it as \textit{average
neighbor connectivity}.
%JDD provides information about the node's proximity and its
%neighborhood since it reveals both the degree distribution $P(k)$ and
%average degree $\bar{k}$~\cite{lessons}.  The average node degree
%thus gives the number of links that on average connect to a
%node.  \subsection{Degree distribution} \subsection{Joint degree
%distribution}


\subsection{Assortativity}

Assortativity is a measure of the likelihood of connection of nodes of similar
degrees~\cite{Newman:2002}. This is usually expressed by means of the
\emph{assortativity coefficient} $r$: assortative networks have $r>0$
(disassortative have $r<0$ resp.) and tend to have nodes that are connected to
nodes with similar (dissimilar resp.) degree.

\subsection{Clustering}

Given node $i$ with $k_i$ links, these links could be involved in at most $k_i(k_i-1)/2$ triangles (e.g. nodes $a\rightarrow{b}\rightarrow{c}\rightarrow{a}$ form a triangle). The greater the number of triangles the greater the clustering of this node. The clustering coefficient, $\gamma{(G)}$, is defined as the average
number of 3-cycles (i.e., triangles) divided by the total number of possible 3-cycles:

$\gamma(G)= \displaystyle 1/N\sum_{i}{\frac{T_i}{k_i(k_i-1)/2}}   ,    k_i\geq 2 $

where $T_i$ is the number of 3-cycles for node $i$, $k_i$ is the
degree of node $i$. We use the distribution of \emph{clustering coefficients} $C(k)$,
which in fact is the distribution of the terms $\frac{T_i}{k_i(k_i-1)/2}$ in the overall summation. This definition of the clustering coefficient gives the same
weight to each triangle in the network, irrespective of the distribution of the node 
degrees.

\subsection{Rich-Club}

The \emph{rich-club coefficient} $\phi(\rho)$ is the ratio of the number of
links in the component induced by the $\rho$ largest-degree nodes to the
maximum possible links $\rho(\rho-1)/2$ where $\rho=1...n$ are the first
$\rho$ nodes ordered by their non-increasing degrees in a network of size $n$
nodes~\cite{Colizza_Flammini_Serrano_Vespignani:2006}.

\subsection{Shortest path}

The shortest path length distribution $P(h)$, as commonly computed using
Dijsktra's algorithm, is the probability distribution of two nodes being at
minimum distance $h$ hops from each other. From the shortest path length
distribution, the average node distance in a connected network is derived as
$\overline{h}=\sum_{h=1}^{h_{\max}}hP(h)$, where $h_{\max}$ is the longest
among the shortest paths between any pair of nodes. $h_{\max}$ is also
referred to as the diameter of a network.

\subsection{Centrality}

Betweenness centrality is a measure of the number of shortest paths passing
through a node or link, a centrality measure of a node or link within a
network. The \emph{node betweenness} for a node $v$ is $B(v)=\sum_{s\neq v\neq
t\in\mathcal{N}}\frac{\sigma_{st}(v)}{\sigma_{st}}$ where $\sigma_{st}$ is the
number of shortest paths from $s$ to $t$ and $\sigma_{st}(v)$ is the number of
shortest paths from $s$ to $t$ that pass through a node $v$
\cite{Holme_Kim_Yoon_Han:2002}. The average node betweenness is the
average value of the node betweenness over all nodes.

Closeness is a another measure of the centrality of a node within a network.
The closeness of a node is the reciprocal of the sum of shortest paths from
this node to all other reachable nodes in a graph.

\subsection{Coreness}

The $l$-core of a network (also known as the $k$-core) is the maximal component in which each node has at
least degree $l$. In other words, the $l$-core is defined as the component of
a network obtained by recursively removing all nodes of degree less than $l$.
A node has coreness $l$ if it belongs to the $l$-core but not to the $(l +
1)$-core. Hence, the $l$-core layer is the collection of all nodes having
coreness $l$. The core of a network is the $l$-core such that the $(l +
1)$-core is empty~\cite{GDEA-566}.

\subsection{Clique}

A clique in a network is a set of pairwise adjacent nodes, i.e. a component
which is a complete graph. The \emph{top clique size}, also known as the graph
clique number, is the number of nodes in the largest clique in a network~\cite{clique}.

\subsection{Spectrum}

Recently, it has been observed that eigenvalues are closely related to almost
all critical network characteristics~\cite{spectralgraph}. For example,
Tangmunarunkit \textit{et al.}~\cite{degreebased} classified network
resilience as a measure of network robustness subject to link failures,
resulting in a minimum balanced cut size of a network. Spectral graph theory
enables studying this problem of network partitioning by using graph's
eigenvalues~\cite{spectralgraph}. In this paper we focus on \emph{graph's
spectrum}, i.e. the set of eigenvalues of the adjacency, the Laplacian or any
other characteristic matrix of a graph. In the graph theory literature, one
usually considers the adjacency or the Laplacian
matrix~\cite{Merris:1995,Cvetkovic_Doob_Gutman_Torgasev:1988}, both which
employ different normalizations and therefore lead to different spectra. Here
we focus on the spectrum of the \emph{normalized Laplacian matrix}%
~\cite{spectralgraph} where all eigenvalues lie between 0 and 2, allowing easy
comparison of networks of different sizes. The normalized graph's spectrum has
been successfully used for tuning the topology generators~\cite{hamedamien}.

